Graphs with maximum degree D at least 17 and maximum average degree less than 3 are list 2-distance (D+2)-colorable

For graphs of bounded maximum average degree, we consider the problem of 2-distance coloring. This is the problem of coloring the vertices while ensuring that two vertices that are adjacent or have a common neighbor receive different colors. It is already known that planar graphs of girth at least 6 and of maximum degree D are list 2-distance (D+2)-colorable when D>=24 (Borodin and Ivanova (2009)) and 2-distance (D+2)-colorable when D>=18 (Borodin and Ivanova (2009)). We prove here that D>=17 suffices in both cases. More generally, we show that graphs with maximum average degree less than 3 and D>=17 are list 2-distance (D+2)-colorable. The proof can be transposed to list injective (D+1)-coloring.

==> rule13.tex <==
\begin{tikzpicture}[scale=0.95] \configtikz \draw node[tnode] (x2)
  [label=left:$x$] {$w$} -- ++(-90:1cm) node[blacknode] (a2)
  [label=left:$a$] {} -- ++(-90:1cm) node[tnode] (y2) [label=left:$y$]
  {\small{$\neg w$ $7^-$}}; \draw (x2) edge [post,bend left] node
  [label=right:$\frac{2}{5}$] {} (a2);
\end{tikzpicture}
